Exploring the Impact of Affine Loop Transformations in Qubit Allocation

Most quantum compiler transformations and qubit allocation techniques to date are either peep-hole focused or rely on sliding windows that depend on a number of external parameters. Thus, global optimization criteria are still lacking. In this paper we explore the synergies and impact of affine loop transformations in the context of qubit allocation and mapping. With this goal in mind, we have implemented a domain specific language and source-to-source compiler for quantum circuits that can be directly described with affine relations. We conduct an extensive evaluation spanning 8 quantum circuits taken from the literature, 3 distinct coupling graphs, 4 affine transformations (including the Pluto dependence distance minimization and Feautrier's minimum latency algorithms), and 4 qubit allocators. Our results demonstrate that affine transformations using global optimization criteria can cooperate effectively in several scenarios with quantum qubit mapping algorithms to reduce the circuit depth, size and allocation time.

==> Makefile <==
# Simple latex makefile
# Author: Martin Kong

PROJ = main
EA = extended-abstract
APPX = appendix
PROJSAN = sanitized-main
PDFLATEX = pdflatex
LATEX = latex
BIBTEX = bibtex
DVIPS = dvips
DVIOPS = -Ppdf -G0 -t letter -o
PSPDF = ps2pdf
PSPDFOPTS = -dPDFSETTINGS=/prepress -dEmbedAllFonts=true
PSPDFOPTS2 = -dPDFSETTINGS=/prepress -dEmbedAllFonts=true

all: paper ea appendix

simple: $(PROJ).tex *.tex figures/* 
	$(LATEX) $(PROJ).tex 
	$(LATEX) $(PROJ).tex 
	$(DVIPS) $(PROJ).dvi;
	$(PSPDF) $(PSPDFOPTS) $(PROJ).ps; 
	while [ `cat $(PROJ).log | grep 'Rerun to get' | wc -l` -gt 0 ]; do \
		echo "latexing ..."; \
		$(LATEX) $(PROJ).tex; \
		$(DVIPS) $(PROJ).dvi; \
		$(PSPDF) $(PSPDFOPTS) $(PROJ).ps; \
	done

paper: $(PROJ).tex *.tex figures/* bib/*
	cat bib/*.bib > allrefs.bib
	$(LATEX) $(PROJ).tex 
	$(LATEX) $(PROJ).tex 
	$(DVIPS) $(PROJ).dvi;
	$(PSPDF) $(PSPDFOPTS) $(PROJ).ps; 
	-makeindex $(PROJ)
	-$(BIBTEX) $(PROJ) 
	while [ `cat $(PROJ).log | grep 'Rerun to get' | wc -l` -gt 0 ]; do \
		echo "latexing ..."; \
		$(LATEX) $(PROJ).tex; \
		$(DVIPS) $(PROJ).dvi; \
		$(PSPDF) $(PSPDFOPTS) $(PROJ).ps; \
	done

ea: $(EA).tex content/*.tex figures/* bib/*
	cat bib/*.bib > allrefs.bib
	$(LATEX) $(EA).tex 
	$(LATEX) $(EA).tex 
	$(DVIPS) $(EA).dvi;
	$(PSPDF) $(PSPDFOPTS) $(EA).ps; 
	-makeindex $(EA)
	-$(BIBTEX) $(EA) 
	$(LATEX) $(EA).tex 
	-$(BIBTEX) $(EA) 
	while [ `cat $(EA).log | grep 'Rerun to get' | wc -l` -gt 0 ]; do \
		echo "latexing ..."; \
		$(LATEX) $(EA).tex; \
		$(DVIPS) $(EA).dvi; \
		$(PSPDF) $(PSPDFOPTS) $(EA).ps; \
	done

appendix: $(APPX).tex content/*.tex figures/* bib/*
	cat bib/*.bib > allrefs.bib
	$(LATEX) $(APPX).tex 
	$(LATEX) $(APPX).tex 
	$(DVIPS) $(APPX).dvi;
	$(PSPDF) $(PSPDFOPTS) $(APPX).ps; 
	-makeindex $(APPX)
	-$(BIBTEX) $(APPX) 
	$(LATEX) $(APPX).tex 
	-$(BIBTEX) $(APPX) 
	while [ `cat $(APPX).log | grep 'Rerun to get' | wc -l` -gt 0 ]; do \
		echo "latexing ..."; \
		$(LATEX) $(APPX).tex; \
		$(DVIPS) $(APPX).dvi; \
		$(PSPDF) $(PSPDFOPTS) $(APPX).ps; \
	done

withfonts: $(PROJ).tex content/*.tex figures/* bib/*
	$(LATEX) $(PROJ).tex 
	-$(BIBTEX) $(PROJ) 
	-makeindex $(PROJ)
	while [ `cat $(PROJ).log | grep 'Rerun to get' | wc -l` -gt 0 ]; do \
		echo "latexing ..."; \
		$(LATEX) $(PROJ).tex; \
		$(DVIPS) $(PROJ).dvi; \
		$(PSPDF) $(PSPDFOPTS) $(PROJ).ps; \
	done

check: 
	pdffonts $(PROJ).pdf

clean: cleanpaper cleanea

cleanpaper: 
	rm $(PROJ).aux $(PROJ).bbl $(PROJ).blg $(PROJ).pdf $(PROJ).log $(PROJ).out  $(PROJ).dvi $(PROJ).ps $(PROJ).xcp

cleanea: 
	rm $(EA).aux $(EA).bbl $(EA).blg $(EA).pdf $(EA).log $(EA).out  $(EA).dvi $(EA).ps $(EA).xcp

cleanappx: 
	rm $(APPX).aux $(APPX).bbl $(APPX).blg $(APPX).pdf $(APPX).log $(APPX).out  $(APPX).dvi $(APPX).ps 
  
  
#$(PROJSAN).aux $(PROJSAN).bbl $(PROJSAN).blg $(PROJSAN).pdf $(PROJSAN).log $(PROJSAN).out


==> codegen.tex <==


The code generation process in \axl~ follows the flow depicted
in Figure \ref{fig:axl-codegen-flow}.
%, and consists of 3 steps,
%which naturally follow from the dynamic aspect of quantum circuits.
Once the polyhedral program representation (SCoP) has been extracted,
the polyhedral scanning process generates the loop and control structure
necessary to visit all the quantum gate operations in the order
defined by the scattering functions (schedules). When possible, we 
leverage the Integer Set Library (ISL) \cite{isl.2010} capabilities
to perform unrolling of the non-degenerate loops in the AST representation
of the program. The next stage builds a binary executable of the program,
and prints out all the gate operations together with the quantum 
register entries being accessed. The output is then used to assemble
the source program for a quantum back-end compiler. 
%For the purpose of this
In this work, we target the OpenQASM (Open Quantum Assembly) 
language \cite{openqasm.arxiv.2017} to produce the experimental data,
and ProjectQ \cite{projectq.2018} to visually render the circuits
(e.g. for debugging purposes). (NOTE: circuits evaluated are included
in the Appendix).

\begin{figure}[htb]
\includegraphics[width=0.95\linewidth]{figures/axl-codegen-flow}
\caption{\label{fig:axl-codegen-flow}AXL code generation flow}
\end{figure}

\iffalse
Prior to the polyhedral scanning process, and in order to generate a complete
quantum program, we construct the set of {\em quantum gate maps} for each
circuit statement. These are extracted from the statement body. In particular,
we generate one {\em affine map} for each distinct quantum gate appearing
in the statement body. The domain of this map is the iteration domain
of the statement. The range of this map will have as many dimensions
as arguments has the gate in question (i.e. 1 for a NOT-gate or 3 for a Controlled-Controlled-NOT).
\fi


==> double-stairs.tex <==

%%\begin{figure}[!htb]
%%\begin{minipage}{0.22\textwidth}
%%\input{generated/cx05-base}
%%\end{minipage}
%%\hspace{5pt}
%%\begin{minipage}{0.22\textwidth}
%%\input{generated/cx05-iss}
%%\end{minipage}
%%\hspace{5pt}
%%\begin{minipage}{0.22\textwidth}
%%\input{generated/cx05-iss-feautrier}
%%\end{minipage}
%%\hspace{5pt}
%%\begin{minipage}{0.22\textwidth}
%%\input{generated/cx05-iss-pluto}
%%\end{minipage}
%%\end{figure}



%\begin{figure}[!htb]
\begin{figure}[!htb]
\begin{minipage}{0.98\linewidth}
\begin{minipage}{0.46\linewidth}
\input{generated/cx05-base}
%\caption{\label{fig:cx05-base} Original}
%\caption{Original}
\end{minipage}%
\hspace{8pt}
\begin{minipage}{0.46\linewidth}
\input{generated/cx05-iss}
%\caption{\label{fig:cx05-iss}ISS only}
%\caption{ISS only}
\end{minipage}
\end{minipage}\\
%\end{figure}
%\hspace{5pt}
\begin{minipage}{0.98\linewidth}
\begin{minipage}{0.46\linewidth}
\input{generated/cx05-iss-feautrier}
%\caption{\label{fig:cx05-iss-feautrier}ISS + Feautrier}
%\caption{ISS + Feautrier}
\end{minipage}%
\hspace{8pt}
\begin{minipage}{0.46\linewidth}
\input{generated/cx05-iss-pluto}
%\caption{\label{fig:cx05-iss-pluto}ISS + Pluto}
%\caption{ISS + Pluto}
\end{minipage}
\end{minipage}
\caption{\label{fig:cx-all}Effects of transformations on double-stairs benchmark:
No transformation (top-left), ISS only (top-right), ISS + Feautrier Algorithm (bottom-left), ISS + Pluto Algorithm (bottom-right)
}
%\end{figure}
\end{figure}


==> driving-example.tex <==

\begin{figure}[htb]
\begin{lstlisting}
param L;
statement S1, S2;

S1 := { t : 0 <= t < L (%) #cX(t,t+2) };
S2 := { t : 0 <= t < L (%) #cY(t,t+3) };

codegen { S1 (+) S2 } with {L=9} apply {iss_stairs,pluto};
\end{lstlisting}
\caption{\label{fig:driving-example} Driving example of an affine quantum program in \axl}
\end{figure}


==> exp-all-topo.tex <==





\paragraph{Individual Analysis with Default Parameters}
We next dissect the behavior of our eight quantum circuits, and show the achieved circuit depth
in Fig.\ref{fig:all:topo}. For each circuit, we cluster the collected circuit depth by
{topology $\times$ allocator}. Each bar represents the mean of 10 repetitions, and include their
corresponding standard desviation. In addition, each cluster is also tagged with the ratio
of highest depth by the lowest one observed. In general, we expect lower variation for the \topogrid~
topology than for the \topomring~ and \topotiled~ topologies.

Turning our attention to the \bpipelined~ circuit. This benchmark represents the swap between 
the top-left qubit ($q0$) and the bottom-right one ($q35$). The circuit initially exhibits 2-way parallelism,
simultaneously starting with the two qubits farthest appart, and morphing into pipelined parallelism
in its steady-state. Each CNOT operation being the input dependence to the operations on two adjacent qubits.
This benchmark clearly benefits from the \trplutomax~ fusion heuristic as it minimizes the maximal 
dependence distance between the producer and consumer instances of a dependence relation.
In a similar spirit, \trplutomin~ consistently achieves the worst circuit depth, as it attempts
to maximize the dependence distance between every pair of CNOT gates.

The \bcheung~ circuit exhibits N-way data-parallelism, N being the number of pipelined CCNOT (Controlled-Controlled NOT) gates found
at the bottom of the circuit. The first CCNOT  of each qubit can be mapped to a distinct
qubit to maximize parallelism and reduce the circuit depth. Intuitively, both the \trfeautrier~ and \trplutomax~ should yield
the highest benefit in terms of circuit depth, since maximizing the number of satisfied dependences 
per schedule dimension equates (for this benchmark) to minimizing the maximal-dependence distance.
The circuit's depth drastically increases with the quality of the qubit
allocator. This is due to the fact that the control qubits for each operation start the closest and
separate as the state evolves. This, in turn, requires more swaps operations to make the qubit
operands adjacent. We note that only qubits with degree 3 or higher are candidates for placement of CCNOT
operations. Therefore, we expect the circuit depth of the \topogrid~ to be shallower than the \topotiled,
and this one also better than \topomring.

The arithmetic adder using the majority and unmajority circuit pattern, \baddermau, exhibits
a highly serial form in its steady-state. The only opportunities for reordering transformations
arise from the potential fusion/distribution of of the CNOT operations with the sequence of CCNOTs
following later. In general terms, we expect the \trplutomax~ to have the highest impact on the circuit depth.
The same observations hold for the \bcuccaro~ adder, which differs from the former in that 
degree of data-parallelism. This translates to much shallower circuits, roughly half the depth of
the \baddermau~ counterparts. It also differs in that \trbase~ and \trplutomin~ typically achieve
the best circuit depth due to the already available parallelism. All four qubit allocators also
benefit from the higher scheduling and placement flexibility of \bcuccaro~ due to the lower number
of CCNOTs (3-operand gates) as well as the presence of CNOT and NOT gates.

Benchmarks \bsum~ and \binit~ \cite{Takahashi:qic.2008} share some similar properties. As both
exhibit distinct and noticeable parallel and serial phases. For instance, \bsum~'s initial 
and \binit~ ending phase
gives a lot of reordering freedom in the scheduling and placement of the CNOT operations.
In contrast, the middle and ending phases of \bsum~ and and initial and middle ones of
\binit~ are mostly serial with stints of pipelined parallelism. In addition, the large and varying separation
between the gate operands induce a higher number of required SWAP operations. These combination
of factors make harder the prediction of the most suitable affine transformatio, making the outcome
highly variable w.r.t to the coupling graph and the qubit allocator. So the overall topological
trends remain.


%% Cheung scaling on 3 topologies
\begin{figure*}[!htb]
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-cheung-depth}
\\
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-cheung-depth}
\\
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-cheung-depth}
\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit depth for \bcheung~ circuit on topologies \topogrid~ (top), \topomring~ (middle) and \topotiled~ (bottom)}
\end{figure*}

Circuit \bcnt~ also shares some features with \bcuccaro. They both have a mix of data-
and pipelined parallelism, with short constant distance (3 or fewer) among the gate operands.
These traits contrast with benchmark \brd~ which exhibits much larger, but constant separation.
However, the latter benefits from a slighter higher degree of pipelined parallelism.
Given these combination of characteristics, we expect \trplutomax~ to be more benefitial 
for \brd~ and \trfeautrier~ to perform best (or close to) for \bcnt. Empirically, both of these
observations and hypotheses hold.








==> exp-pbs-scaling.tex <==

%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/cnt3-5_179-depth}
%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/pipelined-swap-depth}


%%\iffalse
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-cheung-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-cheung-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-cheung-gates}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit gates for \bcheung~ circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%\fi
%%
%%
%%\iffalse
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-cnt3-5_179-depth}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-cnt3-5_179-depth}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-cnt3-5_179-depth}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit depth for \bcnt~ circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-cnt3-5_179-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-cnt3-5_179-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-cnt3-5_179-gates}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit gates for \bcnt~ circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%\fi

\begin{figure*}[!htb]
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-pipelined-swap-depth}
\\
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-pipelined-swap-depth}
\\
\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-pipelined-swap-depth}
\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit depth for \bpipelined~ circuit on topologies \topogrid~ (top), \topomring~ (middle) and \topotiled~ (bottom)}
\end{figure*}

\paragraph{Impact of Circuit Scaling}

To complement our study, we perform a scaling evaluation of circuits \bcheung~ and \bpipelined.
We focus on these benchmarks due to their high regularity and lack of singleton quantum statements
that require more specific scheduling. We test all even numbers of N $\in \{2..12\}$ or until
reaching the number of available qubits. To judge the overall scaling behavior, the last four
bar clusters in each figure represent the \TODO{average} mean of each allocator varying the loop
transformation. 
%It is easy to note the impact of the topology's bisection bandwidth
%for the \bpipelined~ circuit, as the circuit depth largely increases lower bisection bandwidth. 
%This observation holds particularly well for the {\bf wpm} allocator ..
We first center our attention on the \bcheung~ benchmark,
which only utilizes CCNOT gates. This trait makes it fare best on topologies with higher number
of vertices with degree 3 or higher, i.e. \topotiled~(24) and \topogrid~ (32). The impact of
this requirement is notorious on the \topomring~(8) graph, which for N=4 requires a total
of 8 (4 producing and 4 consuming) gates. Past this point the number of quantum swaps operations
introduced by the {\bf wpm} allocator nearly doubles for every increment of 2 on N. Given these resource
restrictions, we now refine our first assessment on this circuit, and expect the \trfeautrier~ transformation to fare best, as it was conceived
as a minimun latency, resource conscious transformation that attempts to provide the highest
(late) scheduling flexibility by satisfying dependences as early as possible. 
Equivalently, we also now expect the \trplutomax~ to induce typically higher circuit depth.
The intution here (in classical loop transformation terms) is that the \trplutomax~ heuristic would amount to an 
outer parallel loop and an inner serial loop, while the \trfeautrier~ transformation would 
make the outerloop serial, thereby exposing more inner parallelism. The general effect of this
trade-off for most qubit allocators is to expose earlier the gate-to-gate dependences. In particular,
this is most benefitial when the allocator makes local decisions using sliding windows.

Changing our focus to the \bpipelined~ circuit, we first note that, unlike the previous benchmark,
this one only consists of CNOT gates. Thus, the number of vertices with degree 3 or higher is
not a limiting factor. This provides more freedom to the qubit allocators. 
In general, the {\bf jku} allocator produces the circuits with the shallowest depth,
outperforming {\bf sabre} in every topology. Nonetheless, 
we highlight that {\bf wpm} in tandem with \trplutomax~ yields results comparable, and at times
better, than {\bf sabre}. This is relevant because {\bf wpm} is $10\times$ faster than {\bf sabre}
and $10\times$ to $15\times$ faster than {\bf jku}. The much improved circuit depth w.r.t
to {\bf wpm}'s impact on other benchmarks is due to an specific feature of \bpipelined~. 
If we divide the circuit into four quadrants, the north-east (NE), north-west (NW), 
south-east (SE) and south-west (SW), and consider this as the four statement to schedule,
we can notice that the NW and SW statements converge in the middle of the circuit. This means
that the underlying qubit allocator would benefit from finding those operations, the ones 
in the middle of the four quadrants, concentrated into a small window of operations. That is
precisely the effect of using \trplutomax~, and leads up to a $2\times$ improvement 
when using {\bf wpm} on the \topotiled~ topology.

It is easy to see the impact of operand separation between both circuits, as the `closer neighbor'
access pattern of \bpipelined~ produces much shallower circuits than \bcheung~ across all topologies.



%%\iffalse
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-pipelined-swap-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-pipelined-swap-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-pipelined-swap-gates}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit gates for \bpipelined circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%\fi
%%
%%\iffalse
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-parity-depth}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-parity-depth}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-parity-depth}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit depth for \bparity circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%
%%\begin{figure*}[!htb]
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/grid/grid-parity-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/mring/mring-parity-gates}
%%\\
%%\includegraphics[width=1.0\linewidth]{figures/scaling-pbs/tiles/tiles-parity-gates}
%%\caption{\label{fig:scaling-pbs}Impact of problem size scaling on circuit gates for \bparity circuit on grid topology (top), multi-ring (middle) and Tiled topologies (bottom)}
%%\end{figure*}
%%\fi


==> exp-swap-scaling.tex <==

\begin{figure*}[!htb]
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/adder-maj-uma-swaps}
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/cheung-swaps}
\\
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/cnt3-5_179-swaps}
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/cuccaro-adder-6qubit-swaps}
\\
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/pipelined-swap-swaps}
\includegraphics[width=0.50\linewidth]{figures/swap-scaling/rca-swaps}
\caption{\label{fig:swap-scaling}Impact of High-Level Loop Transformations on SWAP operations}
\end{figure*}


==> experiments-synthetic.tex <==

%%% 
%%%

%% Synthetic benchmark section starts here

%%%
%%%



\subsection{Evaluation on Synthetic Benchmarks}


%%\begin{table}[t]
%%\caption{\label{tab:iss-benchmark} Index Set Splitting (ISS) 
%%synthetic quantum circuits implemented with \axl}
%%{\center{%
%%{\footnotesize
%%\begin{tabular}{|c|c|c|c|}
%%\hline
%%Benchmark & No.   & Dependence & Gate \\
%%     Name & Stmts & Distance  & Count\\
%%%& No.Used & Reversed \\
%%\hline
%%iss1     &  1 & (4)   & 20 CNOT\\
%%iss2     &  2 & (2,3) & 20 (CNOT + SQRT\_SWAP) \\
%%iss3     &  2 & (6,3) & 20 (CNOT + SQRT\_SWAP) \\
%%%%reverse1a & Reverse and Composition & Synthetic & 2 \\
%%%%reverse1a & Reverse and Composition & Synthetic & 2 \\
%%%%reverse1a & Reverse and Composition & Synthetic & 3 \\
%%%%reverse1a & Reverse and Composition & Synthetic & 3 \\
%%%%reverse1a & Reverse and Composition & Synthetic & 2 \\
%%%%reverse2a & Reverse and Composition & Synthetic & 1 \\
%%%%reverse2b & Reverse and Composition & Synthetic & 1 \\
%%%%reverse2c & Reverse and Composition & Synthetic & 2 \\
%%%%reverse2d & Reverse and Composition & Synthetic & 2 \\
%%\hline
%%\end{tabular}
%%}
%%}
%%}
%%\end{table}



%%% fig 10
%%\begin{figure}[!htb]
%%\includegraphics[width=0.8\linewidth]{figures/syn-iss-dist}
%%%\includegraphics[height=5cm,width=0.98\textwidth]{figures/syn-iss-transfo.pdf}
%%\caption{\label{fig:iss}Synthetic benchmarks for Index Set Splitting Stair Pattern}
%%\end{figure}

%%\textbf{Index Set Splitting (ISS)}
%%We implemented 3 variants to consider the impact of the stair-pattern ISS:
%%{\em iss1}, {\em iss2} and {\em iss3}. The difference among these 3 variants
%%is the number of statements implementing the benchmark and the dependence distance.
%%All three variants perform the same number of CNOT operations, while
%%variants {\em iss2} and {\em iss3} conduct an additional SQRT\_SWAP
%%operation w.r.t {\em iss1}.
%%The summary for this benchmark can be seen in Table \ref{tab:iss-benchmark}.
%%Figure \ref{fig:iss} shows 90 data points, 24 for each of the three iss-variants,
%%and one red bar for the average of every set of 4 window sizes.
%%The 24 data points are obtained from the 4 window sizes used (5, 10, 15 and 20)
%%and the 6 combinations of transformations considered 
%%(base, feautrier, pluto, iss, iss+feautrier, iss+pluto). 
%%We observe 3 distinctive performance trends, which strongly correlate with
%%the maximum dependence distance of each variants, 4, 3 and 6, respectively.

The last set of experiments is designed to show the impact
of both our circuit reversal HLT operation and the effect
of index set splitting.
We evaluate their impact on four variants of a synthetic 
benchmark, {\em reverse2}
The sub-variants evaluated differ in
the manner that statements are composed (See listing in Figure 
%\ref{lst:syn-rev2-source}
\ref{fig:ibmqx20}
and Table \ref{tab:reverse2-desc}).  In this table we can
observe that {\em reverse2b} is the reverse of {\em reverse2a}, and {\em
reverse2d} is the reverse of {\em reverse2c}. 
Their total gate count in principle should be very similar, if not identical.
However, we see that the {\em wpm} and {\em grdy} allocation heuristics
suffer a non-negligible variation of approximately 25 gates. The impact
is much more drastic for the circuit depth on {\em wpm}.
We can also see that the {\em sabre} algorithm appears to be very
sensible to the HLT applied: performing worse for the {\em base},
{\em feautrier} and {\em plutomin}, and much better with the {\em iss\_stairs}
and {\em plutomax}. The ISS was specifically designed for this
scenario, where a circuit exhibits a pipelined pattern, either
decreasing or increasing w.r.t the qubit index value. Thus, 
as the ISS decomposes the affine circuit statement into 2 or
more sub-partitions, the gates associated to the new and independent
sets can be co-scheduled. This shortens the circuit depth.
Lastly, we point out that variants (c) and (d), as they double the
number of original gate operations w.r.t variants (a) and (b), the overall
results on circuit depth and gate count remain proportional.


\begin{figure}[!htb]
\begin{lstlisting}
S1 := { t,i : 0 <= t, t < T, 0 <= i, i < 3 (%) 
  #CY(t,t+2) (+) #CZ(t+i,t+i+3) };
S2 := reverse (S1);
\end{lstlisting}
\caption{\label{lst:syn-rev2-source}Base \axl code for {\em reverse2} synthetic benchmark}
\end{figure}


\begin{table}[!htb]
\caption{\label{tab:reverse2-desc} \axl composition rules for benchmark {\em reverse2}, T=13}
\center{
{\footnotesize
\begin{tabular}{|c|c|c|}
\hline
Sub-variant & Statement Composition & No. of Operations\\
\hline
reverse2a & S1 & 84 \\
reverse2b & S2 & 78 \\
reverse2c & S1 [+] S2 & 78 \\
reverse2d & S2 [+] S1 & 78 \\
\hline
\end{tabular}
}
}
\end{table}




\begin{figure*}[!htb]
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2a-depth}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2a-gates}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2b-depth}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2b-gates}
\\
\vspace{10pt}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2c-depth}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2c-gates}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2d-depth}
\includegraphics[width=0.24\linewidth]{figures/synthetic/topo-grid-syn-reverse2d-gates}
\caption{\label{fig:ibmqx20}Impact of High-Level Loop Transformation on synthetic benchmarks, evaluated on a 36-Qubit Quantum Machine with Grid Topology}
\end{figure*}


==> motiv.tex <==


Quantum computing (QC) has taken a leap forward over the last decade, with
progress in  areas such as theoretical foundations and principles, hardware and
architectures, programming languages and compiler frameworks. While QC systems
are not expected to supplant general-purpose Exascale systems, they are viewed
as having promise as high-performance application-specific accelerators,
capable of making some currently-intractable problems tractable.  Achieving
this promise introduces a wide range of significant challenges.
%In this
%section, we discuss different aspects of introducing QC in heterogeneous
%systems with focus on the roles of compilers and programming languages.

%%The state-of-the-art in Quantum Computing presents two
%%vastly different strategies to define a program. On the one hand,
%%we have the low-level approach of implementing a program
%%in a gate-by-gate basis. This approach is extremely error
%%prone and not scalable for large application. In the other hand,
%%we have tools such as \TODO{Add citations here} synthesize
%%a quantum circuit from an hermitian matrix representing
%%the {\it time evolution operator}. This matrix is decomposed
%%into an extremely large product sequence of {\bf 2-qubit unitary
%%matrices}. Each of the 2-qubit matrices has a direct 
%%mapping to ... Unfortunately, this approach offer very
%%little control of how the matrix is decomposed.

The appeal of QC is its ability to accelerate calculations by leveraging
properties of quantum physics. QC is fundamentally based on {\it qubits},
quantum units of information akin to bits in the classical RAM model.   In
contrast to classical bits that are either 0 or 1, qubit states are linear
combinations of $|0\rangle$ and $|1\rangle$ states, i.e. a $n$-qubit vector can
simultaneously represent $2^n$ states.  This is referred to as {\it
superposition}.  Classical answers are produced in quantum systems by the act
of {\it measurement} of qubits, which causes qubits to lose their superposition
state and collapse probabilistically into one of the component states.  Another
relevant property for quantum systems is {\it entanglement}; namely,  the state
of entangled qubits are inter-dependent, which allows for rich mechanisms for
computing and communicating state. Finally, the {\it no-cloning} property says
that no qubit state can be perfectly copied, so QC systems do not have an
analog for classical "fanout" or accurate data copies.   



\subsection{Quantum Languages: We are not there yet}
\label{sec:background:qlangs}
In the last 15 years, several quantum programming languages have been 
designed and implemented by different institutions and research groups.
Knill's work \cite{knill.lanl.1996} provided some of the first known quantum
pseudo codes, examples and use cases of quantum computing. 
Gay \cite{gay.mscs.2006} and Selinger \cite{selinger.isflp.2004} surveyed
the existing quantum programming languages in the mid 2000s. Since then,
a number of new languages have been proposed 
\cite{quipper.pldi.13,scaffold.tr.2012,openqasm.arxiv.2017,qsharp.rwdslw.2018,projectq.2018,lapets.functionaldsls.2013,qwire.popl.2017}. 

%%In this section, we compare 4 of the most recent languages with 
%%code snippets extracted from the GitHub repositories of OpenQASM, Scaffold,
%%Q\# and ProjectQ . The examples shown are a 5-qubit QFT for OpenQASM and
%%Scaffold (Figure \ref{lst:openqasm-scaffold-qft5}), and the Grover 
%%Search algorithm for Q\# and ProjectQ 
%%(Figure \ref{lst:qsharp-projectQ-search}).
%%These two algorithms embody classic examples from the literature.
%%In particular, QFT is a common building block in several applications,
%%whereas Grover's Search is the classical example where an oracle
%function is used. 
%Most current quantum languages %exhibit different levels
%of abstraction. 
On the lower end of the abstraction spectrum, we have
OpenQASM \cite{openqasm.arxiv.2017}, 
where the user declares classical and quantum registers,
and applies gates to different qubits to perform the task. 
Scaffold \cite{scaffold.tr.2012}
raises the level of abstraction by allowing the definition of 
functions. Figure \ref{lst:scaffold-qft5}
shows a code snippet of the 5-qubit QFT benchmark implemented in Scaffold.
At the core, these approaches are very similar to the assembly level.
The main difference is the ability of applying gates and pre-defined
routines to subsets of a quantum register with control-flow constructs
such as loops and if-then statements.

Similar to Scaffold, Q\# \cite{qsharp.rwdslw.2018} 
and ProjectQ \cite{projectq.2018} also leverage control-flow
constructs to drive the implementation of a program, and applying
gates/functions to quantum registers or to subsets of it (i.e. to
individual qubits). These languages are implemented as extensions
to C\# and Python, where modules can be imported and used. For instance,
ProjectQ uses a circuit engine (variable \texttt{eng}) to perform
the instantiation of qubit registers, and to explicitly generate
the reversed part of the circuit via the \texttt{Uncompute(eng)} call.
Q\# also supports this feature, and allows the user to request
the reversed circuit by invoking the \texttt{Adjoint} or 
\texttt{Auto Adjoint}.

As we see, although the surrounding language (C, C\# or Python)
does raise the level of abstraction and simplifies some tasks, there
still is a substantial semantic gap between the quantum domain
and the state-of-the-art in quantum languages. In particular, all
of the above languages still consider invocation to individual
gates as language statements. This level of abstraction is no different
from writing programs with assembly operations.


%\subsection{\axl Overview}
%\label{sec:axl}



==> polyhedral-flow.tex <==
\begin{tikzpicture}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
%roundnode/.style={ellipse, draw=green!60, fill=green!5, very thick, minimum size=7mm},
%mybox/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
\tikzstyle{mybox}=[very thick, draw=red!60, fill=red!6, rectangle, fill=red!5, minimum size=5mm]
\tikzstyle{myellipse}=[very thick, draw=green!60, fill=green=5, ellipse, fill=green!5, minimum size=7mm]


\node[mybox] (input) {
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
{\begin{varwidth}{\linewidth}
 \boxname{Input\\
 Code
}
\end{varwidth}}
}  
};

\node[myellipse] (extraction) [right=of input] {
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
{\begin{varwidth}{\linewidth}
 \boxname{
Extract\\
Abstractions
}
\end{varwidth}}
}  
};

\node[myellipse] (depanalysis) [right=of extraction] {
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
{\begin{varwidth}{\linewidth}
 \boxname{
Dependence\\ 
Analysis
}
\end{varwidth}}
}  
};

\node[myellipse] (scheduling) [below=of depanalysis] {
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
\boxname{Scheduling}
}
};

\node[myellipse] (codegen) [left=of scheduling]{
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
{\begin{varwidth}{\linewidth}
 \boxname{Code\\
 Generation}
\end{varwidth}}
}  
};

\node[mybox] (output) [left=of codegen]{
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\framebox{
{\begin{varwidth}{\linewidth}
 \boxname{Output\\
 Code}
\end{varwidth}}
}  
};

\draw[->] (input.east) -- (extraction.west);
\draw[->] (extraction.east) -- (depanalysis.west);
\draw[->] (depanalysis.south) -- (scheduling.north);
\draw[->] (scheduling.west) -- (codegen.east);
\draw[->] (codegen.west) -- (output.east);
\end{tikzpicture}


==> qlang-example-qft-openqasm.tex <==

\begin{figure}[!htb]
\begin{minipage}{0.48\textwidth}
%\input{content/example-qft5-scaffold-main}
\input{content/examples/example-qft5-openqasm}
\end{minipage}
\caption{\label{lst:openqasm-qft5} 5-qubit QFT code snippet for OpenQASM}
%\caption{\label{lst:openqasm} OpenQASM 5-qubit QFT code snippet }
\end{figure}


==> qlang-example-qft-scaffold.tex <==

\begin{figure}[!htb]
\begin{minipage}{0.4\textwidth}
%\input{content/example-qft5-scaffold-funcQFT}
\input{content/examples/example-qft5-scaffold}
\end{minipage}
\caption{\label{lst:scaffold-qft5} 5-qubit QFT code snippet Scaffold}
%\caption{\label{lst:openqasm} OpenQASM 5-qubit QFT code snippet }
\end{figure}


==> related-quantum-tech.tex <==

\subsection{Quantum Technologies}
\label{sec:background:qt}
Currently, several competing technologies appear as promising candidates
for quantum computing \cite{ladd.nature.2010,kurizki.nas.2015}. 
Some of these rely  on 
state photon polarization, trapped atoms (e.g. multi-level linear ion traps
or surface ion trap chips), liquid-state nuclear magnetic resonance,
large qubit arrays on solid state hosts (quantum dots and dopants),
and superconducting circuits based on electrical oscillators 
\cite{devoret.science.2013}. All of these technologies offer different 
advantages and disadvantages. Regardless, all of them suffer from the 
\texttt{decoherence problem}, a quantum mechanical destructive process
that causes small amounts of information leakage. Although a number of
Quantum Error Correction (QEC) methods have been proposed, no technology
is impervious to this physical phenomenon. Moreover, QEC is very resource-intensive, imposing a roughly 50X overhead on qubit and operation counts.  As a result, near-term machines are not expected to use QEC at all, and even in the longer-term, a large fraction of quantum resources will be devoted
to QEC 
\cite{knill.nature.2005,oskin.ieee.2002,knill.science.1998}.

In the last years, a number of prototype quantum processors 
\cite{bristlecone.techcrunch.2018,bristlecone.google.2018,ibm-quantum-experience.nature.2017} have been announced, and some made available for public use.  In addition, quantum annealers  are also in use
 (e.g. DWave \cite{wavescalar.tocs.2007,wavescalar.micro.2003}).
The availability of QC machines is opening up a new wave of users and programmers, with a faster feedback cycle as small algorithms can be run on real QC machines.




==> related-synthesis.tex <==

\subsection{Circuit Synthesis}
\label{sec:background:circuits}
%\note{
%  pending to discuss: 
%  sine-cosine decomposition \cite{tucci.arxiv.1999}
%  more cosine-sine decomp \cite{paige.laa.1994}
%  space constraints \cite{parent.arxiv.2015}
%  Williams, genetic algorithm for circuit design \cite{williams.qcqc.1999}, error fidelity, encoding ...
%  }
This section reviews relevant work in the area of circuit 
synthesis for unitary operators. 
Householder \cite{householder.jacm.1958} proposed a method for bringing a
unitary matrix to its triangular form by performing at most $2(n-1)$ square
roots instead of $n(n-1)/2$. 
Deutsch, Barenco and Ekert's seminal paper \cite{deutsch.royalsoc.1995} proved
that almost all n-bit gates, $n > 2$, can represent any computing task.
Barenco et al. \cite{barenco.physreva.1995} showed that a set 
consisting of one-bit quantum gates [U(2)] and the two-bit exclusive-OR
is universal on all unitary operations on arbitrarily many bits $n$ [U($2^n$)].
An important result of this work, initially conjectured but later 
ratified by Knill \cite{knill.arxiv.1995}, was that the number of 2-bit gates required to produce
an arbitrary n-bit operator could be improved from $\Theta(n^{3}4^n)$
to $\Theta(n4^n)$. Using optical devices, Reck and Zeilinger \cite{reck.physrevlet.1994} introduced
a recursive algorithm for factorizing any discrete finite-dimensional
$N \times N$ unitary matrix
into a sequence of two-dimensional beam splitter transformations.
More specifically, any U(N) matrix can be decomposed into a sequence
of U(2) transformations performed on two-dimensional subspaces of the
full N-dimensional Hilbert space. This process is equivalent to decomposing
the U(N) matrix into at most N(N-1)/2 U(2) factors.
\cite{vartiainen.physrevlet.2004}
decreased the lower bound for arbitrary operators to $\Theta(4^n)$
by reordering the basis vectors via Gray code basis and eliminating a
large fraction of control bits.
\cite{mottonen.physreva.2004} applied the Cosine-Sine Decomposition
(CSD) method in a recursive fashion to produce ``uniformly controlled
rotations''. \cite{bergholm.physreva.2005} extended this work for the
synthesis of uniformly controlled one-qubit gates (i.e. that can be 
represented as direct sums of two-dimensional unitary operators)
while attempting to minimize the number of CNOT gates on nearest-neighbor
implementations.
\cite{shende.tcad.2006} established the equivalence between
quantum conditionals and concepts of digital logic such as Shannon 
decomposition of boolean functions. Their work defined quantum conditionals
as multiplexors, and allowed them to generalize CNOT, Toffoli and Fredkin gates.
From the optimization perspective, their work further lowered the
known bounds of circuits for state preparation and arbitrary n-qubit
operators.
Sedl\'ak and Plesch \cite{sedlak.cejop.2008} developed a variant of the Barenco
decomposition algorithm \cite{barenco.physreva.1995} wherein they considered
properties of generalized Toffoli gates such as their commutativity, exchange
of gates with small modifications to one of them, exchange and addition of a
gate, and specific conditions for merging two gates into a single one.
Daskin and Kais \cite{daskin.jocp.2011} used an
evolutionary algorithm to synthesize quantum circuits constrained by circuit
cost (sum of cost of gates) and fidelity error relative to a given matrix
operator. One of the most interesting aspects of their work is the encoding
used to represent basic gates, inputs and outputs. 
More recently, Li, Roberts and Yin \cite{li.ijqi.2013} proposed a unitary
matrix decomposition similar to Barenco's, the difference being that
the U(2) factors (two-level unitaries coined \texttt{P-unitaries}) are 
obtained from permutation vectors. An interesting result of this work
is the large freedom for selecting each P-unitary, as long as the product
of their determinants equals to det(U).
\cite{ross.arxiv.2014,gridsynth.web} developed a fast probabilistic 
scheme for approximating arbitrary
Z-rotations by using an ancilla-free Clifford+T ($\pi/8$ gate) scheme. 
Their tool is
publicly available and can be used as a 
building block for larger compilation sequences.


==> takahashi-circuits.tex <==

\begin{figure}[!htb]
\begin{minipage}{0.45\textwidth}
\begin{lstlisting}
  CCX[0][1][10]
  for (int c8 = 1; c8 <= 2; c8++)
    CX[10][-c8 + 4]
  CCX[2][3][10]
  for (int c8 = 1; c8 <= 2; c8++)
    CX[10][-c8 + 6]
  CCX[4][5][10]
  for (int c8 = 1; c8 <= 2; c8++)
    CX[10][-c8 + 8]
  CCX[6][7][10]
  for (int c8 = 1; c8 <= 2; c8++)
    CX[10][-c8 + 10]
  CCX[2][3][0]
  CCX[4][5][0]
  CCX[6][7][0]
  for (int c1 = 0; c1 <= 1; c1++) {
    if (c1 == 1)
      X[1]
    if (c1 == 0)
      X[1]
    if (c1 == 0) {
      for (int c6 = 0; c6 <= 1; c6++)
        CX[0][-c6 + 9]
      CCX[7][6][0]
      for (int c6 = 0; c6 <= 1; c6++)
        CX[0][-c6 + 7]
      CCX[5][4][0]
      for (int c6 = 0; c6 <= 1; c6++)
        CX[0][-c6 + 5]
      CCX[3][2][0]
      CCX[0][1][9]
      CCX[0][1][8]
      CCX[0][1][7]
      CCX[0][1][6]
      CCX[0][1][5]
      CCX[0][1][4]
    }
  }
  CCX[0][1][3]
  CCX[0][1][2]
\end{lstlisting}
\caption{\label{fig:axl-init5} \axl init\_g5 generated code}
\end{minipage}
\end{figure}

\begin{figure}[!htb]
\begin{minipage}{0.4\textwidth}
\begin{lstlisting}
CX[10][0]
CX[10][1]
CX[10][2]
CX[10][3]
CX[10][4]
CX[10][5]
CX[10][6]
CX[10][7]
CX[0][10]
for (int c7 = 0; c7 <= 1; c7++)
  CX[10][-c7 + 2]
CCX[1][2][10]
for (int c7 = 0; c7 <= 1; c7++)
  CX[10][-c7 + 4]
CCX[3][4][10]
for (int c7 = 0; c7 <= 1; c7++)
  CX[10][-c7 + 6]
CCX[5][6][10]
CCX[1][2][0]
CCX[3][4][0]
CCX[5][6][0]
CX[0][7]
CCX[5][6][0]
CX[0][5]
CCX[3][4][0]
CX[0][3]
CCX[1][2][0]
CX[0][1]
CX[1][2]
CX[3][4]
CX[5][6]
CX[7][8]
CX[9][10]
\end{lstlisting}
\end{minipage}
\caption{\label{fig:axl-sum5} \axl generated C-style code for sum\_5 benchmark}
\end{figure}

\begin{figure}[!htb]
\includegraphics[width=0.95\linewidth]{figures/init_g5-base.pdf}\\
\includegraphics[width=0.95\linewidth]{figures/sum_5-base.pdf}\\
\caption{\label{fig:axl-init-sum-base}Example of circuits written in \axl: init\_g5 (left) and sum\_5 (right)}
\end{figure}

